AT2: Asynchronous Trustworthy Transfers

Many blockchain-based protocols, such as Bitcoin, implement a decentralized asset transfer (or exchange) system. As clearly stated in the original paper by Nakamoto, the crux of this problem lies in prohibiting any participant from engaging in double-spending. There seems to be a common belief that consensus is necessary for solving the double-spending problem. Indeed, whether it is for a permissionless or a permissioned environment, the typical solution uses consensus to build a totally ordered ledger of submitted transfers. In this paper we show that this common belief is false: consensus is not needed to implement of a decentralized asset transfer system. We do so by introducing AT2 (Asynchronous Trustworthy Transfers), a class of consensusless algorithms. To show formally that consensus is unnecessary for asset transfers, we consider this problem first in the shared-memory context. We introduce AT2$_{SM}$, a wait-free algorithm that asynchronously implements asset transfer in the read-write shared-memory model. In other words, we show that the consensus number of an asset-transfer object is one. In the message passing model with Byzantine faults, we introduce a generic asynchronous algorithm called AT2$_{MP}$ and discuss two instantiations of this solution. First, AT2$_{D}$ ensures deterministic guarantees and consequently targets a small scale deployment (tens to hundreds of nodes), typically for a permissioned environment. Second, AT2$_{P}$ provides probabilistic guarantees and scales well to a very large system size (tens of thousands of nodes), ensuring logarithmic latency and communication complexity. Instead of consensus, we construct AT2$_{D}$ and AT2$_{P}$ on top of a broadcast primitive with causal ordering guarantees offering deterministic and probabilistic properties, respectively.

==> sections/algo-shmem.tex <==
%!TEX root = ../main.tex

\section{Consensusless Asset Transfer With \namesh}
\label{sec:result}

In this section, we show that consensus is not necessary for
implementing an asset transfer system.
First, we give a definition of a transfer system as a \emph{sequential type} (\cref{sec:def-sequential}).
Then we show that this type has consensus number \emph{one} by proposing a wait-free implementation called \namesh ~(\Cref{sec:avoiding-consensus}).
Finally, we refine the definition to account for Byzantine, i.e.,
arbitrary, failures (\Cref{sec:def-byz}).

\subsection{Transfer System Specification}
\label{sec:def-sequential}

The state in a transfer system consists of a set of \emph{accounts}.
Each account holds a \emph{balance}, and there is an initial balance set to some pre-defined value.
\footnote{In practice, a mechanism that is external to the system can decide prior to deployment about the initial account balances, similarly to an ICO (Initial Coin Offering).}
The transfer system exports two operations:

\begin{enumerate}
\item \operation{transfer}{(a, b, x)} executes a transfer of amount $x$ from account $a$ to account $b$; and
\item \operation{read}{(a)} returns the balance of account $a$.
\end{enumerate}

We say that the operation \operation{transfer}{(a, b, x)} is \emph{outgoing} for account $a$ and \emph{incoming} for account $b$.
This operation \emph{succeeds}, i.e., returns $\textit{true}$, if and
only if the balance on account $a$ is larger or equal to $x$, in which
case the balance of account $a$ diminishes by $x$ and the balance of account $b$ gains $x$.
Otherwise, if the balance of $a$ is insufficient, the transfer operation \emph{fails}, i.e., returns $\textit{false}$, and the account balances remain unchanged.

We discuss implementations of this sequential
specification in a system of $N$ concurrent \emph{processes}.~\footnote{We use the terms \emph{process}, \emph{participant}, and \emph{replica} interchangeably.}
Our implementation assumes that each account $a$ has a unique \emph{owner} process:
only the owner of $a$ can invoke transfers outgoing from this account.
For simplicity, we assume that each process in the system is the
owner of exactly one account.
The model can be easily extended to allow each process to own multiple accounts.
Trivially, we can do so by introducing a mapping between processes and accounts.
As an alternative solution, we can generate a distinct logical process identity for each account.

\subsection{Transfers Are Easier than Consensus}
\label{sec:avoiding-consensus}

We now show that the consensus number (as defined by Herlihy~\cite{Her91}) of a transfer system is \emph{one}.
An important implication of this result is that an implementation of a transfer
system, as a sequential type, does not need consensus.

Before we discuss the consensus number of the transfer system, we first
 revisit the consensus problem.
Recall that in consensus, each process starts with a private
\emph{input} value and is expected to decide on an \emph{output}
value, so that the following three properties are satisfied:
(1)~no two processes decide on different output values,
(2)~every decided output is an input of some process, and
(3)~every correct process eventually decides on an output.

The \emph{consensus number} of some object type $T$ is the maximal number of processes
that can (wait-free) solve consensus using atomic objects
of type $T$ and atomic registers~\cite{Her91}.
For example, the consensus number of the \textsf{register} type is
\emph{one}: even two processes cannot solve consensus using only
registers~\cite{FLP85,LA87}.

To explain why a transfer system type has consensus number one, let us take a small detour through the shared memory model~\cite{Her91}.
In this model, $N$ concurrent processes communicate by invoking atomic operations
on a collection of shared objects, which, by default, include read-write
registers.
%
For the moment, we assume that processes are subject to \emph{crash}
faults: a faulty process prematurely stops taking steps of its
algorithm. We will come back to the more general model of \emph{Byzantine}
failures in the next section.

Without loss of generality, we can assume that
all processes can access the \emph{atomic-snapshot}
memory (which we build using just read-write registers)~\cite{atomic-snapshot}.
The atomic-snapshot memory is represented as a vector of $N$ memory locations, where
each process is associated with a distinct memory location.
To access the atomic-snapshot memory, processes can use two operations, both of which are atomic: \emph{update} and
\emph{snapshot}.
An \emph{update} operation performed by a process $p$
modifies the value at $p$'s memory location.
The \emph{snapshot} operation simply returns the current state of the whole atomic-snapshot memory.

\begin{figure}[tbp]
\hrule \vspace{1mm}
 {\small
%\setcounter{linenumber}{0}
\begin{tabbing}
 bbb\=bb\=bb\=bb\=bb\=bb\=bb\=bb \=  \kill
Shared variables: \\
\> $A$, atomic snapshot, initially $[\bot,\ldots,\bot]$\\
\\
Local variables: \\
\> $\textit{ops}_p\in (\Pi\times\Pi\times\Nat)^*$\\
\\
Upon \textit{transfer}$(a,b,x)$\\
\nnll\label{line1:tsf:snapshot}\> $S := A.\textit{snapshot}()$\\
\nnll\> \textbf{if} $\textit{balance}(a,S)< x$
\textbf{then}\\
\nnll\label{line1:response-false}\>\> \textbf{return} {\false}\\
\nnll\> $\textit{ops}_p := \textit{ops}_p\cdot(a,b,x)$\\
\nnll\label{line1:tsf:update}\> $A.\textit{update}(\textit{ops}_p)$\\
\nnll\label{line1:response-true}\>\textbf{return} {\true}\\
\\
Upon \textit{read}$(a)$\\
\nnll\label{line1:read:snapshot}\> $S := A.\textit{snapshot}()$\\
\nnll\label{line1:read:response}\> \textbf{return} $\textit{balance}(a,S)$\\

%\vspace{-2mm}
\end{tabbing}
 }
 \hrule
\caption{\namesh: a wait-free \textsf{asset transfer} algorithm using only atomic-snapshot. Code for process $p$.}
\label{fig:waitfree}
\end{figure}

In~\Cref{fig:waitfree} we describe \namesh, a simple algorithm implementing a transfer system using only the atomic-snapshot memory.
Every process $p$ stores the sequence of its outgoing transfers in its
dedicated location in the atomic-snapshot memory.
%

To initiate a new \operation{transfer}{} operation outgoing from its
account, a process $p$ takes a
memory snapshot and then computes, based on this snapshot, its \emph{current balance}.
To compute the balance, process $p$ adds to its initial balance
the sum of all incoming transfers and subtracts the sum of all outgoing transfers found in the returned snapshot.
If the amount of the new transfer does not exceed the
current balance, then process $p$ updates its memory location by
appending the new transfer and returns $\textit{true}$.
Otherwise, the transfer operation fails and returns $\textit{false}$.
A \operation{read}{} operation simply takes a snapshot and
returns the current balance of the account.


%%%%%%%%%% ADI: replaced this correctness arguments with the ones below, since this is too concise & incomplete
% We encourage the interested reader to check~\Cref{app:consnum} for a detailed discussion and the
% proof of correctness of this algorithm.
% Intuitively, every operation is \emph{linearized} (``takes
% effect'')~\cite{herl90linearizability} at the moment it performs a
% memory access (a snapshot or an update).
% Every \operation{read}{} or failed \operation{transfer}{} operation takes
% effect when it takes a memory snapshot.
% Every successful \operation{transfer}{} operation takes effect when it updates
% the memory by appending the new transfer to the sequence of outgoing transfers.

% One can check that the operations put in the order in which they take
% effect respect the sequential specification of a transfer system.
% Indeed, the only potential complication here can come from
% the fact that a successful  \operation{transfer}{} operation by a process $p$ performs two
% memory accesses: a snapshot and an update.
% Indeed, some concurrent successful \operation{transfer}{} operations could
% take effect between these two accesses, affecting $p$'s actual balance.
% However, since $p$ is the only process that can debit its account, all
% such concurrent \operation{transfer}{} operations can only be \emph{incoming} for $p$.
% Thus, between the moment when $p$ takes a memory snapshot and decides that its \operation{transfer}{} operation should
% succeed and the moment when $p$ updates the memory by appending a new
% transfer, $p$'s balance can only grow.
% Therefore, the \operation{transfer}{} operation by $p$ succeeds at the moment $p$ performs its memory update, even if concurrent transfers alter $p$'s balance.
%%%%%%%%%%

\paragraph{Correctness Argument.}
To argue about the correctness of this algorithm, we discuss how each operation is \emph{linearized} in an execution, i.e., the point in an execution when that operation takes effect~\cite{herl90linearizability}.
For every \operation{read}{}, notice that this operation takes effect at the moment when process $p$ takes a memory snapshot.
Likewise, a \operation{transfer}{} operation which fails also takes effect when process $p$ takes a memory snapshot.
A successful \operation{transfer}{} operation is linearized at the moment
when process $p$ updates its memory location to append the new transfer.
%
We claim that in a given execution of this algorithm, all operations (as put in their respective linearization order) respect the sequential specification we have defined earlier (\Cref{sec:def-sequential}).

There is one potential danger for the correctness of the sequential history we
constructed so far.
This can be caused by the interlacing of two successful transfers, as follows.
Consider a transfer $T_1$ initiated by process $p$.
Like any successful transfer, this operation consists of two memory accesses---the first for taking a memory snapshot, and the second access for updating the memory associated with the account of $p$.
It can happen that another transfer, say $T_2$, has the linearization point between the first memory access of $T_1$ and the second memory access of $T_1$.
%
%

In such a case of concurrent transfers, the balance which process $p$ computes based on the first memory access of $T_1$ can be outdated, because $T_2$ affects this balance.
Recall, however, that only process $p$ can use the account to initiate outgoing (debit) transfers.
For this reason, the only operations which may change the balance of $p$'s account are \emph{incoming} transfers, so operation $T_2$ must be an incoming transfer to $p$.
When operation $T_1$ is linearized, the balance in the account of $p$ can be outdated, but this balance can only be larger than the balance which $p$ computed.
This corner-case poses no problem to the correctness of the algorithm because the balance of $p$ cannot drop below zero.
Therefore, the actual balance of $p$ when its transfer
is linearized can only by higher than it was computed earlier.
\needsrev{We encourage the interested reader to check~\Cref{app:consnum} for a detailed discussion and the
proof of correctness of this algorithm.}

Having constructed an implementation of our \namesh transfer system only on top of an atomic snapshot proves that \namesh is not stronger than atomic snapshot.
The atomic snapshot object has consensus number \emph{one}.
Hence, the transfer system must also be of consensus number \emph{one}.

This algorithm can be easily extended to implement a transfer system
for a distributed setting where processes communicate via
reliable message-passing, assuming that a majority of processes
are correct~\cite{ABD95}.
In the next section, we consider the issue of Byzantine failures.


\subsection{Securing Against Byzantine Faults}
\label{sec:def-byz}

We now return to the message-passing model where some processes may
behave in a Byzantine manner.
In this setting, Byzantine processes may attempt to double-spend, i.e., initiate
transfers which cannot be justified by the balance in their accounts.
We therefore refine our transfer system specification to ensure
that the transfer system behaves correctly towards \emph{benign} processes,
regardless of the behavior of Byzantine ones.
We say that a process is benign if it respects the algorithm and can only fail by crashing.


Informally, we require that every system execution appears to benign processes as a
correct sequential execution.
As a result, no benign process can be a victim of
a double-spending attack.

Moreover, we require that this execution respects the real-time order among
operations performed by benign processes~\cite{Her91}: when such an
operation completes it should be visible to every future
operation invoked by a benign process.
%
%

For the sake of efficiency, in our algorithm (\cref{sec:algo}), we
slightly relax the last requirement---while still preventing
double-spending.
\needsrev{@NSDI review D: ``is this a fundamental limitation of your approach?...''}
We require that \emph{successful} \operation{transfer}{} operations invoked
by benign processes constitute a legal sequential history that preserves the real-time
order.
A \operation{read}{} or a failed \operation{transfer}{} operation invoked
by a benign process $p$ can be
``outdated'', it can be based on a stale state of $p$'s balance.
%
Informally, one can view the system requirements as \emph{linearizability}~\cite{herl90linearizability}
for successful transfers and \emph{sequential consistency}~\cite{Attiya1994} for failed
transfers and reads.
%
As progress (liveness) guarantees, we require that every operation
invoked by a correct process eventually completes.
One can argue that this relaxation incurs little impact on the system's utility, as long as all incoming transfers
are eventually applied.
\needsrev{In~\Cref{app:byz} we give a more precise discussion of this specification.}


==> sections/appendices/gossip-analysis.tex <==
%!TEX root = ../../main.tex

\section{Full analysis: \erg}
\label{appendix:erganalysis}

In this appendix, we evaluate the security and complexity of \erg.

\subsection{Security}

We start by verifying that \erg\ satistifes both \textbf{no duplication}, \textbf{integrity} and $0$-\textbf{validity}, independently of $G$.

\begin{theorem}
\label{theorem:ergnoduplication}
\erg\ satisfies no duplication.
\begin{proof}
Procedure $dispatch$ explicitly checks (\cref{line:ergcheckdelivered}) if the variable $delivered$ is equal to $\bot$ before delivering any message. Before a message is delivered (\cref{line:ergdeliver}), $delivered$ is updated to a value different from $\bot$ (\cref{line:ergsetdelivered}). Therefore a correct process only delivers one message.
\end{proof}
\end{theorem}

\begin{theorem}
\label{theorem:ergintegrity}
\erg\ satistifes integrity.
\begin{proof}
Upon receiving a {\tt Gossip} message, a correct process checks its $signature$ against the public key of the designated sender $\sigma$ (\cref{line:ergchecksignature}). Moreover, if $\sigma$ is correct, it only signs $message$ when broadcasting (\cref{line:ergbroadcast}). Since we assume that cryptographic signatures cannot be forged, this implies that the message was previously broadcast by $\sigma$.
\end{proof}
\end{theorem}

\begin{theorem}
\label{theorem:ergvalidity}
\erg\ satisfies 0-validity.
\begin{proof}
Upon broadcasting a message $m$, a correct sender calls the procedure $dispatch(m, sign(m))$ (\cref{line:ergbroadcast}). Since $delivered$ is initialized to $\bot$, this immediately results in the delivery of $m$ (\cref{line:ergdeliver}).

Since the validity property is satisfied deterministically, \erg\ satisfies  $\epsilon$-validity for $\epsilon = 0$.
\end{proof}
\end{theorem}


We now compute, given the parameter $G$, the $\epsilon$-\textbf{totality} of \erg. To this end, we first prove some preliminary lemmas.

\begin{lemma}
\label{lemma:gossipreciprocation}
Let $\rho$ and $\pi$ be two correct processes, let $\rho$ be in $\pi$'s gossip sample. Then $\pi$ is eventually in $\rho$'s gossip sample.
\begin{proof}
A gossip sample is updated only upon initialization (\cref{line:erginitializesample}) or when a {\tt GossipSubscribe} message is received (\cref{line:ergupdatesample}).

If $\pi$ selected $\rho$ upon initialization, then it also sent it a {\tt GossipSubscribe} message (\cref{line:ergsubscribe}). Since Byzantine network scheduling can only finitely delay the messages between correct processes, $\rho$ eventually receives $\pi$'s message (\cref{line:ergreceivesubscribe}) and adds $\pi$ to its gossip sample.

If $\pi$ received a {\tt GossipSubscribe} message from $\rho$, then (\cref{line:ergsubscribe}) $\rho$ selected $\pi$ upon initialization, which means that $\pi$ is already in $\rho$'s gossip sample.
\end{proof}
\end{lemma}

\begin{definition}[Correct gossip network]
Let $\pi$, $\rho$ be two correct processes, let $\pi \leftrightarrow \rho$ denote the condition \emph{$\rho$ is eventually in $\pi$'s gossip sample}. \cref{lemma:gossipreciprocation} proves that
\begin{equation*}
    \rp{\pi \leftrightarrow \rho} \Leftrightarrow \rp{\rho \leftrightarrow \pi}
\end{equation*}

We define \textbf{correct gossip network} to be the undirected graph
\begin{equation}
    \mathbb{G} = \rp{\Pi_C, \cp{\rp{\pi, \rho} \in \Pi^2_C \mid \pi \leftrightarrow \rho}}
\end{equation}
\end{definition}

\begin{lemma}
\label{lemma:gossipconnectedness}
If the correct gossip network is connected, then \erg\ satisfies totality.
\begin{proof}
We start by noting that a correct process eventually delivers a message (\cref{line:ergdeliver}) if and only if it eventually sets $delivered$ to a value different from $\bot$ (\cref{line:ergsetdelivered}).

Let $\pi$ be a correct process for which eventually $delivered \neq \bot$. Upon setting $delivered \leftarrow (m \neq \bot)$, $\pi$ sends $m$ to all the processes in its gossip sample (\cref{line:ergforward}). Moreover, upon receiving a {\tt GossipSubscribe} message \emph{after} setting $delivered \leftarrow m$, $\pi$ replies with $m$ (\cref{line:ergcatchup}).

Therefore, every correct process that is eventually in $\pi$'s gossip sample eventually satisfies $delivered \neq \bot$. If $\mathbb{G}$ is connected, then a path exists in $\mathbb{G}$ between $\pi$ and every other correct process, and they all eventually satisfy $delivered \neq \bot$, i.e., they deliver a message.
\end{proof}
\end{lemma}

From \cref{lemma:gossipconnectedness} it follows that \erg\ satisfies $\epsilon$-totality if the probability of $\mathbb{G}$ being disconnected is at most $\epsilon$.

\begin{lemma}
\label{lemma:gossipconnectionprobability}
In the limit $N \rightarrow \infty$, $\mathbb{G}$ is a $G\rp{C, p}$ Erdős–Rényi graph, with
\begin{equation*}
    p = 1 - \rp{1 - \frac{G}{N}}^2
\end{equation*}
\begin{proof}
It is a known result that, for large samples and small probabilities, a binomial distribution converges to a Poisson distribution:
\begin{equation*}
    \lim_{\substack{N \rightarrow \infty \\ Np = \text{const}}} \qp
    {
        \bin{N}{p}{n} = {N \choose n} p^n \rp{1 - p}^{N - n}
    }
    =
    \qp
    {
        \frac{\rp{Np}^n}{n!}e^{-Np} = \pois{Np}{n}
    }
\end{equation*}
therefore, in the limit $N \rightarrow \infty$,
\begin{equation}
    \label{equation:poissontobinomial}
    \pois{G}{n} \simeq \bin{N}{\frac{G}{N}}{n}
\end{equation}

As we discussed in \cref{subsection:ergalgorithm}, a gossip sample $\mathcal{G}$ is initialized upon initialization (\cref{line:erginitializesample}) by first sampling a value $\bar G$ from a $\text{Pois}\qp{G}$ distribution, then selecting $\bar G$ distinct processes from $\Pi$ with uniform probability.

Let $\pi \in \Pi_C, \rho \in \Pi$, let $\mathcal{G}^{in}_\pi$ be $\pi$'s initial gossip sample, let $q = G/N$. By the law of total probability, and using \cref{equation:poissontobinomial}, we have for large $N$
\begin{eqnarray*}
\prob{\rho \in \mathcal{G}^{in}_\pi} &=& \sum_{\bar G = 0}^N \rp{\prob{\rho \in \mathcal{G}^{in}_\pi \mid \bar G} \prob{\bar G}} = \\
&=& \sum_{\bar G = 0}^N \rp{\frac{\bar G}{N} \pois{G}{\bar G}} \simeq \sum_{\bar G = 0}^N \rp{\frac{\bar G}{N} \bin{N}{q}{\bar G}} = \\
&=& \sum_{\bar G = 0}^N \rp{\frac{\bar G}{N} {N \choose {\bar G}} q^{\bar G}\rp{1 - q}^{N - \bar G}} = \\
&=& \sum_{\bar G = 0}^N \rp{\frac{\bar G}{N} \frac{N!}{\bar G! \rp{N - \bar G}!} q^{\bar G} \rp{1 - q}^{N - \bar G}} = \\
&=& \sum_{\bar G = 1}^N \rp{\frac{\rp{N - 1}!}{\rp{\bar G - 1}!\rp{N - \bar G}!} q q^{\bar G - 1}\rp{1 - q}^{N - \bar G}} = \\
&=& q \sum_{\bar G' = 0}^{N - 1} \rp{\frac{\rp{N - 1}!}{\bar G'! \rp{N - 1 - \bar G'}!} q^{\bar G'} \rp{1 - q}^{N - 1 - \bar G'}} = \\
&=& q \sum_{\bar G' = 0}^{N - 1} \bin{N - 1}{q}{\bar G'} = q
\end{eqnarray*}

Let $\rho_1, \ldots, \rho_R$ be distinct processes, with $R \leq N$. Similar calculations yield
\begin{equation}
    \label{equation:independentgossipsampling}
    \prob{\rho_1 \in \mathcal{G}^{in}_\pi, \ldots, \rho_R \in \mathcal{G}^{in}_\pi} = q^R
\end{equation}

\cref{equation:independentgossipsampling} proves that every process $\rho \in \Pi$ has an independent probability $q$ of being in $\mathcal{G}^{in}_\pi$. Since for any two $\pi, \xi \in \Pi_C$ we have
\begin{equation*}
    \rp{\pi \leftrightarrow \xi} \Leftrightarrow \rp{\pi \in \mathcal{G}^{in}_\xi \vee \xi \in \mathcal{G}^{in}_\pi}
\end{equation*}
we can derive the probability $p$ of any two correct processes being connected:
\begin{equation}
    \label{equation:gossipconnectionprobability}
    p = 1 - \rp{1 - q}^2 = 1 - \rp{1 - \frac{G}{N}}^2
\end{equation}

Therefore, following \cref{equation:independentgossipsampling,equation:gossipconnectionprobability}, $\mathbb{G} = G(C, p)$ is an Erdős–Rényi graph with $H$ nodes and $p$ probability of connection between any two nodes.
\end{proof}
\end{lemma}

\cref{lemma:gossipconnectionprobability} allows us to compute the $\epsilon$-totality of \erg, given $G$.

\begin{theorem}
\label{theorem:ergtotality}
\erg\ satisfies $\epsilon_t$-totality, with $\epsilon_t$ bound by
\begin{equation}
    \label{equation:ergtotalitysecurity}
    \epsilon_t \leq \sum_{k = 1}^{C/2} \rp{{C \choose k}\rp{1 - p}^{k\rp{C - k}}}
\end{equation}
\begin{proof}
It follows immediately from \cref{lemma:gossipconnectionprobability} and a known result \cite{phasetransitions} on the connectivity of Erdős–Rényi graphs.
\end{proof}
\end{theorem}

\cref{figure:ergsecurity} shows the $\epsilon$-security of \erg, as a function of the gossip sample size ($G$), the fraction of Byzantine failures ($f$) and the size of the system ($N$).


==> sections/appendices/shmem.tex <==
%!TEX root = ../../main.tex

% \appendix

\section{Consensus number of a Payment System}
\label{app:consnum}


\subsection{System model}
\label{app:system-model}

\myparagraph{Processes and cryptographic primitives.}
We consider a set $\Pi$ of $N$ asynchronous processes that communicate through
reliable message-passing.
%
Every process is provided with a private-public key pair.

\myparagraph{Object types.}
A sequential object type is defined as a tuple
$T=(Q,q_0,O,R,\Delta)$, where $Q$ is a set of states, $q_0\in Q$ is an
initial state, $O$ is a set of operations, $R$ is a set responses and
$\Delta\subseteq Q\times O \times Q \times R$ is a relation
that associates a state and an operation to a set of
possible new states and corresponding responses.
Here we assume that $\Delta$ is total on the first two elements,
i.e., for each state $q\in Q$ and each operation in $o\in O$, some
transition to a new state is defined, i.e., $\exists q'\in Q,\; r\in
R$: $(q,o,q',r)\in \Delta$.

A \emph{history} is a sequence of invocations and responses and a
sequential history is a history that starts with an invocation and in
which every invocation is immediately followed with a response.
A \emph{sequential history} $o_1,r_1,o_2,r_2,\ldots$, where $\forall i\ge
1, o_i\in O,\; r_i\in R$, is \emph{legal} with respect to type
$T=(Q,q_0,O,R,\Delta)$ if there exists a
sequence of states $q_1,q_2,\ldots$ of states in $Q$ such that
$\forall i\geq 1$, $(q_{i-1},o_1,q_i,r_i)\in \Delta$.
%The \emph{sequential specification} of $T$ is the set of all sequential
%histories it accepts.

\myparagraph{Implementations.}
An \emph{implementation} of an object type $T$ is a distributed algorithm that,
for each process and invoked operation, prescribes the actions that the process needs to
take to perform it.
%In our case, the actions are accesses to shared atomic objects or   \textit{broadcast}
%primitives, processing of \textit{receive} events and returning
%responses to the invoked operations.
%
An \emph{execution} of an implementation is a sequence of
\emph{events}: invocations and responses of operations, \emph{send}
and \emph{receive} events, or atomic accesses to shared abstractions. The sequence of events at every process
must respect the algorithm assigned to it.
%A process is called \emph{faulty} in an infinite execution if
%stops before performing an event prescribed by its algorithm;
%otherwise it is called \emph{correct}.

%In the implementation, every process $p_i$ is assigned with an \emph{algorithm} $A_i$, an
%automaton that defines the actions $p_i$ needs to perform when it
%receives an input from its application or receives a message from
%another process.

\myparagraph{Failures.}
Processes are subject to \emph{Byzantine} failures. A process is
Byzantine if it deviates from the algorithm it is assigned, either by
halting prematurely, in which case we say that the process is \emph{crashed}, or performing actions
that are not prescribed by its algorithm, in which case we say that
the process is \emph{malicious}.
We assume that malicious processes can perform arbitrary actions,
except for ones that involve subverting cryptographic primitives (e.g. inverting secure hash functions).

A process is called \emph{faulty} if it is either crashed or malicious.
A process is \emph{correct} if it is not faulty and
\emph{benign} if it is not malicious. Note that every correct process
is benign, but not necessarily vice versa.

In a system with Byzantine processes, we assume that a fraction of less than $N/3$ processes can be malicious.

\myparagraph{Linearizability and sequential consistency.}
We assume that no process invokes a new operation before receiving a
response for the previous one.
For each pattern of invocations, the implementation produces a
\emph{history}, i.e., the sequence of distinct invocations and responses,
labelled with process identifiers and unique sequence numbers.

A projection of a history $H$ to process $p$, denoted $H|p$ is the
subsequence of elements of $H$ labelled with $p$.
An invocation $o$ by a process $p$ is \emph{incomplete} in $H$ if it is not followed by a
response in $H|p$.
A history is \emph{complete} if it has no incomplete invocations.
A \emph{completion} of $H$ is a history $\bar H$ that is identical to
$H$ except that every incomplete invocation in $H$ is either removed or
\emph{completed} by inserting a matching response somewhere after it.

A \emph{sequentially consistent} implementation of $T$ ensures that for every
history $H$ it produces, there exists a completion $\bar H$ and a
legal sequential history $S$ such that for all processes $p$, $\bar H|p=S|p$.
%In other words, the operations in $H$ are consistent to
%legal sequential history

A \emph{linearizable}  implementation, additionally, preserves the
real-time order between operations.
Formally, an invocation $o_1,r_1$ \emph{precedes} an
invocation $o_2$ in $H$, denoted  $o_1\prec_H o_2$, if $o_1$ is
complete and the corresponding response $r_1$ precedes $o_1$ in $H$.
Note that $\prec_H$ stipulates a partial order on invocations in $H$.
%
A linearizable implementation of $T$ ensures that for every history $H$ it produces, there exists a completion $\bar H$ and a
legal sequential history $S$ such that (1)~for all processes $p$, $\bar H|p=S|p$ and (2)~$\prec_H\subseteq\prec_S$.

A (sequentially consistent or linearizable) implementation is
\emph{$t$-resilient} if, under the assumption that at most $t$
processes crash, it ensures that every invocation performed by a
correct process is eventually followed by a response.
In the special case when $t=n-1$, we say that the implementation is
\emph{wait-free}.

In reasoning about correctness of an implementation, we cannot impose
restrictions on the behavior of malicious processes.
Thus, in the system with malicious processes,
given an object type, a history $H$ is \emph{sequentially consistent}
if there exists a
legal sequential history $S$ such that for all \emph{benign} processes $p$, $H|p=S|p$.
%
Note that $S$ may include arbitrary entries coming from malicious
processes.
%\pknote{Distinguish between honest (benign) and malicious?}
Similarly, a history is \emph{linearizable}
if it is sequentially consistent and $S$
respects the precedence order among operations issued by benign processes.
%\pknote{Prove that no linearizable algorithm exists with $f\geq n/2$?}

\myparagraph{Consensus number.}
In the  \emph{consensus} problem, each process starts with a private
\emph{input} value and is expected to decide on an \emph{output}
value, so that the following three properties are satisfied:
\begin{enumerate}
\item[(1)] no two processes decide on different output values,
\item[(2)] every decided output is an input of some process, and
\item[(3)] every correct process eventually decides on an output.
 \end{enumerate}

The \emph{consensus number} of a type $T$ is the maximal number of processes
that can (wait-free) solve consensus using atomic (linearizable) objects
of type $T$ and atomic registers.
For example, the consensus number of the \textsf{register} type is
one: even two processes cannot solve consensus using only
registers~\cite{FLP85,LA87}.

\subsection{Object Type of a Payment System}
\label{app:obj-type}

The \textsf{payment system} object type
%associated with a set of \emph{accounts} $\A$
is defined as a tuple $(Q,q_0,O,R,\Delta)$, where:

\begin{itemize}

\item The set of states $Q$ is the set of all possible maps
  $q:\;\Pi\to\Nat$. Intuitively, each state of the objects assigns
  each account with its \emph{balance}.

\item The initialization map  $q_0:\;\Pi\to\Nat$ assigns the initial
  balance to each account. We assume the initialization map to be fixed for the rest
  of the paper.

\item Operations and responses of  the type are defined as $O=\{\textit{pay}(a,b,x):\; a,b\in\Pi,\,
  x\in\Nat\}\cup\{\textit{read}(a):\;a\in\Pi\}$ and
  $R=\{\true,\false\}\cup\Nat$.

 \item For a state $q\in Q$, an operation $o\in O$, a response
   $r\in R$ and a new state $q'\in Q$, the tuple $(q,o,q',r)\in\Delta$
   if and only if one of the following conditions is satisfied:

  \begin{itemize}

     \item $o=\textit{pay}(a,b,x)$: $q(a)\geq x$, $q'(a)=q(a)-x$, $q'(b)=q(b)+x$ (and all other
       accounts are as in $q$), and $r=\true$;

     \item $o=\textit{pay}(a,b,x)$: $q(a)< x$, $q'=q$, and $r=\false$;

     \item o=$\textit{read}(a)$: $q=q'$, $r=q(a)$.

   \end{itemize}

  \end{itemize}


In other words, operation $\textit{pay}(a,b,x)$ \emph{succeeds} if and only if the source
account $a$  has enough balance, and if it does, $x$ is transferred
from $a$ to the destination account $b$.
%
An $\textit{pay}(a,b,x)$ operation is called \emph{outgoing} for
$a$ and \emph{incoming} for $b$; respectively, the $x$ units are called   \emph{outgoing} for
$a$ and \emph{incoming} for $b$.
A transfer is \emph{successful} if its corresponding response is \emph{true} and \emph{failed} if its corresponding response is \emph{false}.

Operation $\textit{read}(a)$ simply returns the balance of $a$ and
leaves the accounts untouched.

%Let $\mu:\;\Pi\to\Pi$ be the \emph{ownership map} associating each account with a distinct
%process. We require that only $\mu(a)$, the owner of account $a\in \Pi$, is
%allowed to perform $\textit{pay}$ operations on it.
%
%% In a system in which all processes are benign (correct or failing by
%% crashing), we assume that a process $p$ invokes
%% $\textit{pay}(a,.,.)$ or $\textit{read}(a)$ only if $a=p$.
%% Further, in a system assuming the presence of malicious processes, the
%% requirement only applies to benign processes.
%
We assume that every benign process $p$ is \emph{well-formed}: (1)~it
only invokes operations $\textit{read}(a)$ and
$\textit{pay}(a,*,*)$ such that $a=p$ and (2)~it never invokes a new operation before obtaining a response from a previous one.

While not requiring malicious processes to be well-formed, a cryptographic proof of a process invoking an operation on an
account that the process does not own can be used as a proof of misbehavior.

%% \subsection{Banking in a Byzantine environment}
%% %

%% \needsrev{
%% We discuss two implementations of the \textsf{banking} data type.
%% %
%% The first one is a conventional linearizable implementation.
%% %
%% The second one ensures sequential consistency for \emph{updates}, i.e.,
%% successful pay operations and a specific level of \emph{stale}
%% consistency for \emph{read-only} operations, i.e., reads and
%% failed transfers.
%% }


\subsection{Consensus Number of Payment System}
\label{app:consensus-number}

We show that the \textsf{payment system} object type can be
implemented in the \emph{wait-free} manner using only read-write
registers.
%
Thus, the type is of consensus number $1$.

The implementation is described in Figure~\ref{fig:waitfree}.
The idea is very simple.
The $n$ processes share an atomic snapshot object~\cite{atomic-snapshot}.
Every process $p$ is associated with a distinct location in the object
where it stores the sequence of all successful {\transfer} operations
it executed so far.
%

Recall that the atomic-snapshot (AS) memory is represented as a vector of $n$
shared variables, where each process $p$ is associated with a distinct
position $p$. The memory can be accessed with two atomic operations: \emph{update} and
\emph{snapshot}. An \emph{update} operation performed by $p$
modifies the value at position $p$  and a \emph{snapshot} returns the current state of the vector.

To read the balance of an account $a$, the process simply takes a snapshot $S$ and
computes the sum of incoming units minus the sum of all outgoing
units, we  denote this number by $\textit{balance}(a,S)$.
As we argue below, the result is guaranteed to be non-negative,
i.e., the operation does make sense with respect to the type specification.

To perform $\transfer(a,b,x)$, a process $p$, the owner of $a$, takes a snapshot and
computes the balance of $a$ based on all operations that
\emph{concern} $a$ (transfer units from or to $a$).
%
If the amount to be transferred does not exceed the balance of $a$
computed based on operations in the snapshot, the operation is added
to the list of $p$'s operations in the snapshot object via an
\textit{update} operation and $\true$ is returned.
Otherwise, the operation returns $\false$.

Note that security concerns are not central for us now.
In particular, every process has a complete view of all the accounts,
regardless of whether it owns them or not.
%

\begin{theorem}
  \label{th:waitfree}
  The \textsf{payment system} object type can be wait-free implemented in the
  read-write shared memory model.
\end{theorem}
\begin{proof}
  Fix an execution $E$ of the algorithm in Figure~\ref{fig:waitfree}.
   As, atomic snapshots can be wait-free implemented in the read-write
   shared memory model~\cite{atomic-snapshot}.
  As every operation only involves a finite number of atomic-snapshot
  accesses, every process completes each of the operations it invokes
  in a finite number of its own steps.

Let $\textit{Ops}$ be union of all complete operations and
all {\transfer} operations that \emph{completed} the update operation
(line~\ref{line1:tsf:update}) in $E$ (the atomic snapshot operation
has been linearized).
%
Let $H$ be the history of $E$.
%
We determine a completion of $H$ and, for each $o\in\textit{Ops}$, we define a linearization point as
`follows:

\begin{itemize}

  \item If $o$ is a {\read} operation, it linearizes at the
    linearization point of the snapshot operation in
    line~\ref{line1:read:snapshot}.


  \item   If $o$ is a {\transfer} operation that returns {\false},
    it linearizes at the linearization point of the snapshot operation in
    line~\ref{line1:tsf:snapshot}.

 \item   If $o$ is a {\transfer} operation completed in
   line~\ref{line1:tsf:update},  it linearizes at the
    linearization point of the update operation in
    line~\ref{line1:tsf:update}.
    If $o$ is incomplete in $H$, we complete it with response $\true$.

\end{itemize}

Let $\bar H$ be the resulting complete history and let $L$ be sequence
of complete operations of $\bar H$ places in the order of their
linearization points in $E$.
%
Note that, by the way we linearize operations, the linearization of a
prefix of $E$ is a prefix of $L$.

Now we show that $L$ is legal and, thus, $H$ is
linearizable.
%
We proceed by induction, starting with the empty (trivially, legal)
prefix of $L$.
%
Let $L_{\ell}$ be the legal prefix of the first $\ell$ operation and
$op$ be the $(\ell+1)$st operation of $L$.
Let $op$ be invoked by process $p$.
%
The following cases are possible:

\begin{itemize}

\item $op$ is a {\read}$(a)$: the snapshot taken at the linearization point of $op$
  contains all successful payments concerning $a$ in $L_{\ell}$. By
  the induction hypothesis, the resulting balance is non-negative.

\item $op$ is a failed {\transfer}$(a,b,x)$: the snapshot taken at the linearization point of $op$
  contains all successful payments concerning $a$ in $L_{\ell}$. By
  the induction hypothesis, the resulting balance is non-negative.

\item  $op$ is a successful  {\transfer}$(a,b,x)$:  by the algorithm,
  before the linearization point of $op$, process $p$ took a snapshot.
  Let $L_{k}$, $k\leq\ell$, be the prefix of $L_{\ell}$ that only
  contain operations linearized before the moment of time when the
  snapshot was taken by $p$.

  We observe that includes a \emph{subset} of all incoming payments on $a$ and
  \emph{all} outgoing payments on $a$ in $L_{\ell}$. Indeed, as $p$
  is the owner of $a$ and only the owner of $a$ can perform outgoing
 payments on $a$, all outgoing payments in $L_{\ell}$ were
  linearized before the moment $p$ took the snapshot within $op$.
  Thus, $\textit{balance}(a,L_k)\geq \textit{balance}(a,L_{\ell})$.

  By the algorithm, as $op={\transfer}(a,b,x)$ succeeds, we have
  $\textit{balance}(a,L_k)\geq x$.
  Thus, $\textit{balance}(a,L_{\ell})\geq x$ and the resulting balance
  in $L_{\ell+1}$ is non-negative.

\end{itemize}

Thus $H$ is linearizable.
\end{proof}

\begin{corollary}\label{cor:consensus}
The \textsf{payment system} object type has consensus number $1$.
\end{corollary}


\section{Defining a Byzantine Fault-Tolerant Payment System}
\label{app:byz}

In the message-passing context with Byzantine processes, we propose a
relaxed consistency definition that will allow us to build an
efficient implementation.
The implementation ensures linearizability to successful pay
operations, while reads and failed payments are provided with a
weaker consistency property.
Intuitively, every operation performed by a benign process $p$ that does not change the state of the banking object
is consistent with the ever-growing $p$'s local history\footnote{The \emph{local history} of a process $p$ is the subset of the global history observed by $p$.} which might
possibly miss some of the complete incoming payments.
One can argue that this relaxation incurs very little impact on the
utility of the banking application, as long as all incoming payments
are \emph{eventually} accounted for.

%Intuitively, by doing so we relax
%the requirement that complete operations \emph{take effect} in their
%precedence order. It can be argued that the requirement is not central
%for banking applications.

More precisely, we require that in every history $H$ produced by the implementation,
each correct process completes all of its operations.
Moreover, we expect that the \emph{successful} payments in $H$ are
compatible with the same legal sequential execution. In particular, regardless of the
behavior of Byzantine processes, we exclude the problem of double
spending: there is no way a faulty process can spend more money than
its account allows.
Additionally, we require that
reads and unsuccessful payments performed by every benign process $p$ are
compatible with \emph{some} (possibly depending on the process) legal
sequential history.
Also, if $p$ and $q$ are correct, then every successful payment from
$p$ to $q$ is eventually included in $q$'s local history.
%All operations of $p_i$ ``make sense'' for some
%ordering of operations $H$.

\begin{definition}
\label{def:banking-relaxed}
 Let $E$ be any execution of an implementation and $H$ be
the corresponding history.
Let $\textit{ops}(H)$ denote the set of operations in $H$ that were
executed by correct processes in $E$.
%
A \emph{relaxed} banking object guarantees that
each invocation issued by a correct process is followed by a
matching response in $H$, and that there exists $\bar H$,  a completion of $H$, such that:

\begin{enumerate}

\item[(1)] Let $\bar H^{t}$ denote the sub-history of
  successful payments of $\bar H$ performed by correct processes and
  $\prec_{\bar H}^t$ be the subset of $\prec_{\bar H}$ restricted to
  operations in $\bar H^{t}$.
  %we call such a history
%\emph{transfer-only}.
  Then there exists a legal sequential history $S$ such that (a)~for every correct process
$p$, $\bar H^{t}|p=S|p$ and (b)~$\prec_{\bar H}^t\subseteq\prec_S$.
 %with respect to the
 % specification of \textsf{banking}.

\item[(2)] For every correct process $p$, there exists a legal sequential history $S_p$
  such that:

  \begin{itemize}

  \item $\textit{ops}(\bar H) \subseteq \textit{ops}(S_p)$, and

  \item $S_p|p= \bar H |p$.

  \end{itemize}

\end{enumerate}
%
\end{definition}

Notice that property~(2) implies  that every update in $H$ that
affects the account of a correct process $p$ is eventually included in
$p$'s ``local'' history and, therefore, will reflect
reads and pay operations subsequently performed by $p$.
%[[PK already said
%It is possible, however, that $p_i$ may temporarily miss some of the
%transfers affecting its accounts and, as a result, local views of
%different accounts may not be compatible with the same sequential
%history.
%]]
